Communication-Efficient and Byzantine-Robust Distributed Learning with Error Feedback

We develop a communication-efficient distributed learning algorithm that is robust against Byzantine worker machines. We propose and analyze a distributed gradient-descent algorithm that performs a simple thresholding based on gradient norms to mitigate Byzantine failures. We show the (statistical) error-rate of our algorithm matches that of Yin et al.~\cite{dong}, which uses more complicated schemes (coordinate-wise median, trimmed mean). Furthermore, for communication efficiency, we consider a generic class of $\delta$-approximate compressors from Karimireddi et al.~\cite{errorfeed} that encompasses sign-based compressors and top-$k$ sparsification. Our algorithm uses compressed gradients and gradient norms for aggregation and Byzantine removal respectively. We establish the statistical error rate for non-convex smooth loss functions. We show that, in certain range of the compression factor $\delta$, the (order-wise) rate of convergence is not affected by the compression operation. Moreover, we analyze the compressed gradient descent algorithm with error feedback (proposed in \cite{errorfeed}) in a distributed setting and in the presence of Byzantine worker machines. We show that exploiting error feedback improves the statistical error rate. Finally, we experimentally validate our results and show good performance in convergence for convex (least-square regression) and non-convex (neural network training) problems.

==> err-feedback.tex <==
\section{Distributed Learning with Error Feedback}
\label{sec:error_feedback}

In this section, we analyze the role of error feedback \cite{errorfeed} in distributed learning. We modify the problem setup slightly. Here, our goal is to solve the following optimization problem

\begin{align*}
\min_w F(w) = \frac{1}{m} \sum_{i=1}^m F_i(w),
\end{align*}
where $F_i(.)$ is the local loss function at machine $i$. Note that the above optimization problem is a deterministic one, where the data points in the worker nodes are fixed. Consequently, solving this problem does not imply any generalization guarantee.


\begin{algorithm}[t!]
  \caption{Distributed Compressed Gradient Descent with Error Feedback}
  \begin{algorithmic}[1]
 \STATE  \textbf{Input:} Step size $\gamma$, Compressor $\mathcal{Q}(.)$
 \STATE \textbf{Initialize:} Initial iterate $w_0$, $e_i(0) = 0$ $\forall$ $i \in [m]$ \\
  \FOR{$t=0,1, \ldots, T-1 $}
  \STATE \underline{Central machine:} sends $w_t$ to all worker \\
  \textbf{for $i \in [m]$ do in parallel}\\
  \STATE \underline{$i$-th worker machine:}
    \begin{itemize} 
        \item computes $p_i(t) = \gamma \nabla F_i(w_t) + e_i(t)$
        \item sends $\mathcal{Q}(p_i(t))$ to the central machine
        \item computes $e_i(t+1) = p_i(t) - \mathcal{Q}(p_i(t))$
    \end{itemize}
  \STATE  \underline{At Central machine:}
    \begin{itemize}
        \item $w_{t+1} = w_t - \frac{1}{m}\sum_{i=1}^m \mathcal{Q}(p_i(t))$
    \end{itemize}
  \ENDFOR
  \end{algorithmic}\label{alg:err_feed}
\end{algorithm}

 We also assume that $\alpha =0$, meaning there is no adversary in the system. The details of the algorithm we use to solve the above optimization problem is given in Algorithm~\ref{alg:err_feed}. The worker nodes adds the error in compression to the local gradient in subsequent iteration. Adding error feedback somewhat \emph{corrects} the error in compression and guides the trajectory towards the optimization problem without compression. In \cite{stich2018sparsified,errorfeed}, the advantages of error feedback is analyzed for a non-distributed setting. Here, we extend the results to a distributed setting. 

\subsection{Theoretical Guarantee}

Here, we show the convergence of Algorithm~\ref{alg:err_feed}. We concentrate only for non-convex smooth $F(.)$. We start with the following assumption.

\begin{assumption}
\label{asm:lip}
The local loss functions $F_i(.)$ are $L$ Lipschitz for all $ i \in [m]$.
\end{assumption}

We have the following rate of convergence of Algorithm~\ref{alg:err_feed} to a critical point of the loss function $F(.)$.
\begin{theorem}
\label{thm:err_feed}
Suppose that $F(.)$ is $L_F$ smooth and Assumption~\ref{asm:lip} holds. Also, $\mathcal{Q}(.)$ is a $\delta$ compressor. With $\gamma < \frac{1}{L_F}$, we have

\begin{align*}
    \min_{t = 0,.,T}\|\nabla F (w_t) \|^2  & \leq \frac{F(w_0) - F(w^*) }{ \gamma (T+1)  (\frac{1}{2} - \frac{L_F \gamma}{2})}  + \frac{4\gamma^2 L_F^2 L^2 (1-\delta)}{\delta^2  (\frac{1}{2} - \frac{L_F \gamma}{2})}.
\end{align*}

\end{theorem}

\begin{remark}
Note that the first term in the above equation comes from optimizing a non-convex function and it is completely independent of $\delta$. The second term comes from compression. If $\delta =1$ (no compression), the second term vanishes.
\end{remark}

\begin{remark}
Choosing $\gamma = \frac{1}{L_F \sqrt{T+1}}$, we 
%obtain
%\small
%\begin{align*}
%    \min_{t = 0,.,T}\|\nabla F (w_t) \|^2 & \leq C_1 \frac{L_F (F(w_0) - F^*)}{\sqrt{T+1}} + C_2 \frac{L_F L^2 (1-\delta)}{\delta^2 (T+1)}.
%\end{align*}
%\normalsize
notice that, the second term decreases at a much faster $(\mathcal{O}(1/T))$ than the first term $(\mathcal{O}(1/\sqrt{T})$). Hence, we get the compression \emph{for free} in this setting.
\end{remark}
\begin{remark}
Optimizing for the step size, we obtain $ \gamma = \mathcal{O}(\delta^2/(1-\delta)T)^{1/3}$ and correspondingly,\\
 $ \min_{t = 0,.,T}\|\nabla F (w_t) \|^2 \leq \mathcal{O}( \frac{(1-\delta)^{1/3}}{\delta^{2/3} T^{2/3}})$.
\end{remark}

\begin{remark}
In the experiments (Section~\ref{sec:experiment}), we observe that Algorithm~\ref{alg:err_feed} works even in the presence of the Byzantine worker machines. 
\end{remark}

==> newexp.tex <==
\section{New Experiment}
'More number of Byzantine machines': Keeping the same setup of the paper, we run experiments and observe that our algorithm can tolerate more than $33 \%$ Byzantine machines, and show the convergence of our algorithm. The plots are shown in Figure 2 (a) (for least squares regression) and Figure 2 (b) (for feed-forward neural net on MNIST data, with a deterministic shift in label attack). Although in theory, we see a trade-off between compression and the number of Byzantine machines, in practice this turns out not to be a bottleneck.

'More Byzantine machines with proposed attack': We implement the attack proposed by the reviewer with more than $33 \%$ Byzantine machines, set $\epsilon = 0.9 $, along with the compression scheme of KRSJ19. We observe that our algorithm still manages to tackle this scenario and converges. It is shown for both regression (Figure 3 (a)) and neural net (Figure 3 (b)) settings.
\begin{figure}[h!]%
    \centering
    \subfloat[]{{\includegraphics[width=6cm]{rev1_sgn.png} }}%
    \qquad
    \subfloat[]{{\includegraphics[width=6cm]{rev1_trim.png} }}%
    \caption{ }%
    \label{rev1}%
\end{figure}

\begin{figure}[h!]%
    \centering
    \subfloat[]{{\includegraphics[width=6cm]{rev2_det_reg.png} }}%
    \qquad
    \subfloat[]{{\includegraphics[width=6cm]{rev2_det_nn.png} }}%
    \caption{ }%
    \label{rev2_det}%
\end{figure}

\begin{figure}[h!]%
    \centering
    \subfloat[]{{\includegraphics[width=6cm]{rev2_neg_reg.png} }}%
    \qquad
    \subfloat[]{{\includegraphics[width=6cm]{rev2_neg_nn.png} }}%
    \caption{ }%
    \label{rev2_det}%
\end{figure}
